Multiplicative deconvolution under unknown error distribution

We consider a multiplicative deconvolution problem, in which the density $f$ or the survival function $S^X$ of a strictly positive random variable $X$ is estimated nonparametrically based on an i.i.d. sample from a noisy observation $Y = X\cdot U$ of $X$. The multiplicative measurement error $U$ is supposed to be independent of $X$. The objective of this work is to construct a fully data-driven estimation procedure when the error density $f^U$ is unknown. We assume that in addition to the i.i.d. sample from $Y$, we have at our disposal an additional i.i.d. sample drawn independently from the error distribution. The proposed estimation procedure combines the estimation of the Mellin transformation of the density $f$ and a regularisation of the inverse of the Mellin transform by a spectral cut-off. The derived risk bounds and oracle-type inequalities cover both - the estimation of the density $f$ as well as the survival function $S^X$. The main issue addressed in this work is the data-driven choice of the cut-off parameter using a model selection approach. We discuss conditions under which the fully data-driven estimator can attain the oracle-risk up to a constant without any previous knowledge of the error distribution. We compute convergences rates under classical smoothness assumptions. We illustrate the estimation strategy by a simulation study with different choices of distributions.

==> _app1.tex <==
%======================================================================================================================
%                                                                 
%
% ======================================================================================================================
\pagebreak
\section{Important Inequalities}\label{a:prel}
%

% --------------------------------------------------------------------
% <<Re \ref{re:diff_fun}>>
% --------------------------------------------------------------------

In this section we are summarising the most important inequalities used frequently in this paper. \\
We start with \textit{Talagrand's Inequality}, which is well-known and where the proof can be found for example in \cite{Talagrand1996}.
\begin{lem}[Talagrand's inequality]\label{lem: Talagrand}  Let
	$X_1,\dots,X_n$ be independent $\mathcal Z$-valued random variables and let $\bar{\nu}_{h}=n^{-1}\sum_{i=1}^n\left\{\nu_{h}(X_i)-\E\left(\nu_{h}(X_i)\right) \right\}$ for $\nu_{h}$ belonging to a countable class $\{\nu_{h},h\in\mathcal H\}$ of measurable functions. Then,
	\begin{align}
	\IE\left[(\sup_{h\in\mathcal H}|\overline{\nu}_h|^2-6\Psi^2)_+\right]\leq \Const \left[\frac{\tau}{n}\exp\left(\frac{-n\Psi^2}{6\tau}\right)+\frac{\psi^2}{n^2}\exp\left(\frac{-K n \Psi}{\psi}\right) \right]\label{tal:re1} 
	\end{align}
	with numerical constants $K=({\sqrt{2}-1})/({21\sqrt{2}})$ and $C>0$ and where
	\begin{equation*}
	\sup_{h\in\mathcal H}\left\{\sup_{z\in\mathcal Z}\left\{|\nu_{h}(z)|\right\}\right\}\leq \psi,\qquad \E\left[\sup_{h\in \mathcal H}|\bar{\nu_{h}}|\right]\leq \Psi,\qquad \sup_{h\in \mathcal H}\left\{\frac{1}{n}\sum_{i=1}^n \Var(\nu_{h}(X_i))\right\}\leq \tau.
	\end{equation*}
\end{lem}
\begin{rem}
	Keeping the bound Eq. \ref{tal:re1}  in mind, let us
	specify particular choices $K$, in fact $K\geq \tfrac{1}{100}$.
	The next bound is now an immediate consequence, 
	\begin{align}
	&	\IE\left[(\sup_{h\in\mathcal H}|\overline{\nu}_h|^2-6\Psi^2)_+\right]\leq \Const \left(\frac{\tau}{n}\exp\left(\frac{-n\Psi^2}{6\tau}\right)+\frac{\psi^2}{n^2}\exp\left(\frac{-n \Psi}{100\psi}\right) \right)\label{tal:re3} 
	\end{align}
	In the sequel we will make use of the slightly simplified bounds Eq. \ref{tal:re3} rather than Eq. \ref{tal:re1}.
\end{rem}

The next lemma provides \textit{Petrov Inequality} to upper bound sums of independent variables by its moments. The corresponding proof can be found in \cite{Petrov}.
\begin{lem}\label{lem:Petrov}(Petrov)
    Let $\{X_{i}\}_{i\in\nset n}$ be i.i.d. random variables, such that $\IE[X_{1}^q]<\infty$ for some $q\in\pRz$. Then
    \begin{equation}
        \E\bigg[\bigg(\sum_{i\in\nset n}(X_{i}-\E[X_{i}])\bigg)^q\bigg]\leq C(q)\cdot n^{\frac{q}{2}}\E[X_{1}^q].
    \end{equation}
\end{lem}


\begin{lem}\label{lem:Nagalev}(Nagalev)
    Let $(X_{i})_{i\in\nset n}$ be i.i.d. random variables, such that $\E[X_{1}^q]<\infty$ for some $q\in\pRz$. Then
    \begin{equation}
        \forall \varepsilon\in\pRz:\,\Pz\bigg[\bigg|\sum_{i\in\nset n}(X_{i}-\E[X_{i}])\bigg|\geq\varepsilon\bigg]\leq C(q)\cdot \frac{n^{q+1}}{\varepsilon^q}\E[X_{1}^q].
    \end{equation}
\end{lem}
\begin{pr}\label{pr: Process Estimate}
Let $\Theta\subseteq\Rz$ finite and $\ell:=\log(|\Theta|)\lor 1$ and $(Z_i)_{i\in\nset n}$ be an i.i.d. sequence. Let $\phi:\Rz^2\to\Rz$ be a measurable function such that $\E[|\phi(Z_1,t)|]<\infty$ for any $t\in\Theta$. Define the random centered function $\widehat{\Phi}_n:\Theta\to\Rz$ by 
\begin{equation}
    \forall t\in\Theta:\,\widehat{\Phi}_n(t):=n^{-1}\sum_{i\in\nset n}\phi(Z_i,t)-\E[\phi(Z_1,t)].
\end{equation}
Further assume that $\sigma_{\phi,q}:=\E[\sup_{t\in\Theta}|\phi(Z_1,t)|^q]^{\frac{1}{q}}<\infty$ for an $q>2$. Le $x_n$ be a sequence such that $\inf_{n>n_o}\sqrt{n}\frac{x_n}{\ell^{\frac{3}{2}}}>0$ for some $n_o\in\Nz$. Then we have 
\begin{equation}
    \Pz[\sup_{t\in\Theta}|\widehat{\Phi}_n(t)|\geq x_n]\leq C_q\sigma_{\phi,q}^q\frac{n^{1-q}\ell^{\frac{q}{2}}}{x_n^{q}}+C_q\exp\bigg(-\frac{C_qnx_n^2}{\sigma_{\phi,q}^2}\bigg)
\end{equation}
\end{pr}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "_MUDUNER"
%%% End:


==> _packages.tex <==
%EJS Packages
\RequirePackage[OT1]{fontenc}
\RequirePackage{amsthm,amsmath}
\RequirePackage[numbers]{natbib}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{mathrsfs} 
\usepackage{stmaryrd} % for \llbracket and \rrbracket
\usepackage{dsfont} % for mathds
\usepackage{bm} %bm notation
\usepackage{ctable}
\usepackage[singlelinecheck=false,labelsep=none]{caption}
\usepackage{float}
\usepackage{cleveref}

==> _theoremstyle.tex <==
\startlocaldefs
\numberwithin{equation}{section}
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{pr}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{co}[thm]{Corollary}

\theoremstyle{remark}
\newtheorem{rem}{Remark}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{il}{Illustration}[section]
\newtheorem{notation}{Notation}[section]
\newtheorem{ass}{Assumption}[section]
\renewcommand{\theass}{A.\Roman{ass}}
\endlocaldefs


%%% cleverref muss ans ende
\crefname{pr}{Proposition}{Propositions}
\crefname{co}{Corollary}{Corollaries}
\crefname{thm}{Theorem}{Theorems}
\crefname{lem}{Lemma}{Lemmata}
\crefname{ass}{Assumption}{Assumptions}
\crefname{section}{Section}{Sections}
\crefname{appendix}{Appendix}{Appendices}
\crefname{subsection}{Subsection}{Subsections}
\crefname{paragraph}{Paragraph}{Paragraphs}
\crefname{table}{Table}{Tables}
\crefname{rem}{Remark}{Remarks}
\crefname{notation}{Notation}{Notations}
\crefname{definition}{Definition}{Definitions}
